BayesIMP: Uncertainty Quantification for Causal Data Fusion

While causal models are becoming one of the mainstays of machine learning, the problem of uncertainty quantification in causal inference remains challenging. In this paper, we study the causal data fusion problem, where datasets pertaining to multiple causal graphs are combined to estimate the average treatment effect of a target variable. As data arises from multiple sources and can vary in quality and quantity, principled uncertainty quantification becomes essential. To that end, we introduce Bayesian Interventional Mean Processes, a framework which combines ideas from probabilistic integration and kernel mean embeddings to represent interventional distributions in the reproducing kernel Hilbert space, while taking into account the uncertainty within each causal graph. To demonstrate the utility of our uncertainty estimation, we apply our method to the Causal Bayesian Optimisation task and show improvements over state-of-the-art methods.

==> 99_paper_content/07_conclusions.tex <==
\section{Future work}
In the coming weeks we intend to apply our proposed KCGP on real-world data to round up the paper. In particular we are looking into health care data at the moment (other suggestions would be very welcome). Moreover, current experiments with Case 3 do not seem to indicate good uncertainty estimates due to the crude approximation methods that we are using. We will further investigation into Case 3 after finishing up the real-world examples. 

\jef{avoid the term data fusion with sth else}

==> 99_paper_figs/03_new_methodology.tex <==
\section{Two-staged Causal Gaussian Processes}


\begin{minipage}{\textwidth}
\begin{minipage}[b]{0.49\textwidth}
\centering
%\includegraphics[width=1\textwidth]{99_paper_figs/Causal_Exp-Page-19 (1).jpg}
\includegraphics[width=1\textwidth]{99_paper_figs/2SCGP2.png}
\captionof{figure}{The two-staged causal learning problem}
\end{minipage}
\hfill
\begin{minipage}[b]{0.49\textwidth}
\centering
\begin{tabular}{lcc}
\toprule
METHODS                    &  Stage 1   & Stage 2 \\ 
\midrule
Causal Embedding \cite{singh2020kernel}     & KRR & KRR \\
CMP (OURS) & KRR & GP \\
BayesCME (OURS)           & GP  & KRR \\
2SCGP (OURS)            & GP  & GP  \\
\bottomrule
\end{tabular}
\captionof{table}{Summary of our proposed methods}
\end{minipage}
\end{minipage}


\label{sec: method}
Now that we have briefly gone over the necessary background material, we are now ready to present our proposed methodologies. Recall $\EE[T|Y]=f(Y)$ for some RKHS function $f$, thus the expectation can be expressed in terms of kernel mean embeddings:
\begin{align}
    \mathbb{E}[T|do(X)=x] &= \mathbb{E}[f(Y)|do(X)=x]
                          = \langle f, \mu_{Y|do(X)=x} \rangle \label{intergral_mean_embedding}
\end{align}
by using the Representer Theorem: $f(y) = \sum \alpha_i \langle \phi_y(y_i), \phi_y(y) \rangle$ and Eq.\ref{def: causal_emb}.

%Note that the final expression in Eq.\ref{intergral_mean_embedding} does not contain any sampling nor conditional density estimation steps. Instead our formulation models all densities in the RKHS and this allows us to estimate $\mathbb{E}[T|do(X)=x]$ through the notion of kernel mean embeddings. Contrary to sampling methods that use GPs, we do not have any assumptions on the distributions between the nodes such as for example uni-modality.

% Recall that our goal is to quantify the uncertainty when estimating the following expectation:
% \begin{align}
%     \EE[T|do(X)=x] &= \int f(y) p(y|do(X)=x)dy \\
%                   &= \langle f, \mu_{Y|do(X)=x}\rangle
% \end{align}
Recall the setup from Fig \ref{fig: setup1}. There are two distinct quantities to estimate, $f$ and $\mu_{Y|do(X)=x}$. We aim to learn the causal conditional mean embedding $\mu_{Y|do(X)=x}$ using $D_C=\{(x_i, z_i, y_i)\}_{i=1}^N$ and the integrand $f$ from $D_E=\{(\tilde{y}_j, t_j)\}_{j=1}^M$.


% \begin{table}[t]
% \center
% \caption{Summary of non parametric methods to estimate $\EE[T|do(X)]$. Note that $\mu_{Y|do(X)}$ is learnt from $\cD_C$ and $f$ from $\cD_E$.}
% \vspace{0.1cm}
% \begin{sc}
% \begin{tabular}{lccc}
% \toprule
% METHODS                    &  $\mu_{Y|do(X)}$   & $f$   & Uncertainty \\ 
% \midrule
% CAUSAL MEAN EMBEDDING \cite{singh2020kernel}     & KRR & KRR & \text{X}             \\
% CAUSAL MEAN PROCESS (OURS) & KRR & GP  & \checkmark             \\
% BLCME-KRR (OURS)           & GP  & KRR &    \checkmark         \\
% BLCME-GP (OURS)            & GP  & GP  &    \checkmark         \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{table}

% \begin{table}[t]
% \begin{center}
% \begin{medium}
% \begin{sc}
% \resizebox{12.3cm}{!}{%
% \begin{tabular}{lccc}\label{table:Our_methods}
% \toprule
% Methods & $\mu_{Y|do(X)}$ & $f$ & Uncertainty \\
% \midrule
% Causal Mean Embedding \cite{singh2019kernel}  & KRR & KRR & \text{X} \\
% Causal Conditional Mean Process (ours) & KRR & GP & \checkmark \\
% BLCME-KRR (ours) & GP & KRR & \checkmark \\
% BLCME-GP (ours) & GP & GP & \checkmark \\
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{medium}
% \end{center}
% \caption{Summary of the our proposed methods, where $\mu_{Y|do(X)}$ is learnt from $\cD_C$ and $f$ from $\cD_E$.}
% \end{table}

We introduce the following 3 algorithms that estimate $\EE[T|do(X)=x]$ while taking into account uncertainty across different datasets. Note that \textsc{Causal Conditional Mean Process} and \textsc{BLCME-KRR} are introduced as necessary intermediate steps for deriving \textsc{BLCME-GP}, which is our main algorithm of the paper.
%We introduce 3 novel ways to estimate the above expectation while obtaining an uncertainty estimates (See Table \ref{table:Our_methods} for a summary):

 \begin{itemize}
     \item \textbf{\textsc{Causal Mean Process}}: Firstly, we will consider the case where we estimate $f$ using a GP and $\mu_{Y|do(X)=x}$ using vector-valued kernel ridge regression (V-KRR). This allows us to take into account the uncertainty from $\cD_E$ by modelling the relationship between $Y$ and $T$ using a GP. Note that integration is linear and hence it is easy to see that when defining a GP on $f$ the resulting integral will also be Gaussian, see Proposition \ref{proposition: CausalCMP}.
     \item \textbf{\textsc{BLCME-KRR}}: Next, we consider the case where we estimate $f$ using a KRR and $\mu_{Y|do(X)=x}$ using V-GP. Here we first introduce a novel Bayesian version of CMEs, and further extend it to the causal embeddings $\mu_{Y|do(X)=x}$ introduced in section 3. Modelling the causal embedding with V-GP allows us to take into account the uncertainty from the causal graph $\cD_C$. %Note that estimating the causal CME $\mu_{Y|do(X)=x}$ using a V-GP is novel, and has to the best of our knowledge not been done before. 
     
%     Viewing $\mu_{Y|do(X)=x}$ using a V-GP allows us to take into account the uncertainty when modelling the causal graph using $\cD_C$. %Here again we note that integration is linear and hence the resulting integral is also Gaussian as shown in \ref{proposition: f is krr cme is gp}.
     \item \textbf{\textsc{BLCME-GP}}: Finally, we combine the above two situations to take into account all uncertainties in both datasets, $\cD_C$ and $\cD_E$. We estimate $f$ using a GP and $\mu_{Y|do(X)=x}$ using a V-GP. 
    %  However, there are certain drawbacks to this formulation which we will describe in more detail in Section \ref{sec: BLCME-GP}.
 \end{itemize}

Note that Chau et al. [add ref] studied this integral in the non-causal setting, i.e. conditional densities instead of \textit{do}-densities, for a very specific deconditioning problem [add ref]. In particular, they introduced the \textsc{Conditional Mean Process} which allows them to place a prior over the conditional means directly, accounting for uncertainty in $f$. In this paper, we adapt their formulation for the causal setting and therefore obtain the \textsc{Causal Conditional Mean Process}.

\subsection{Causal Mean Process}
The \textsc{Causal Mean Process} gives us a way to propagate uncertainty in $f$ to $\EE[T|do(X)=x]$. Intuitively, we are exploiting the fact that integration and Gaussianity are linear and therefore $\int f(y) p(y|do(X)=x)dy$ will also result in a Gaussian. Hence below, we derive the corresponding mean and covariance for the resulting integral.

\begin{proposition}[\textbf{Causal Mean Process}] \label{proposition: CausalCMP}
Given dataset $D_C=\{(x_i, z_i, y_i)\}_{i=1}^N$ and $D_E=\{(\tilde{y}_j, t_j)\}_{j=1}^M$, if $f$ is a GP learnt from $D_E$, then the integral $\int f(y) p(y|do(X)=x)dy$ is a GP defined on the treatment variable $X$ with the following mean and covariance (given the posterior $f$),
\begin{align}
    m_1(x) &= {\bf t}^\top (K_{\tilde{Y}\tilde{Y}}+ \lambda_f I)^{-1}K_{\tilde{Y}Y}(K_{\Omega} +  \lambda_{cme}I)^{-1} \Phi_{\Omega}(x) \\
    \kappa_1(x, x') &= \Phi_{\Omega}(x)^\top (K_\Omega + \lambda_{cme} I)^{-1} \bar{K}_{\tilde{Y}\tilde{Y}} (K_\Omega + \lambda_{cme} I)^{-1} \Phi_{\Omega}(x)
\end{align}
where $K_{\tilY\tilY} = \Phi_{\tilY}^\top\Phi_{\tilY}, K_{\tilY Y} = \Phi_{\tilY}^\top \Phi_{Y}$ and $\bar{K}_{\tilde{Y},\tilde{Y}}$ is the posterior covariance of $f$ evaluated at $\tilde{y}$. $\Omega$ is the set of variables that are conditioned in obtaining the expression for the do densities as specified above. 
\end{proposition}
However, since $f$ only consider uncertainty exists in $D_E$, we need to develop a methodology that allows us to quantify uncertainty also while learning the causal mean embedding from $D_C$.

To this end, we introduce the novel Bayesian Learning of CMEs using vector-valued GP regression. We firstly, introduce the conditional version for simplicity and then introduce the causal version which follows immediately. Now, we are able to estimate $\langle f, \mu_{Y|do(X)=x}\rangle$, where $f$ is a KRR and $\mu_{Y|do(X)=x}$ is estimated using a V-GP which we call Bayesian Learning of Causal Conditional Mean Embeddings (BLCCME-KRR) (Section \ref{sec:BLCME-KRR}). Given that we are now in a Bayesian setup we also derive the corresponding marginal likelihood, which can thus be optimized for the hyperparameter learning. This is reminiscent of \cite{flaxman2016bayesian}, however they only consider the marginal case, whereas we extended it to the conditional as well as causal case, which is non trivial. At last, to incorporate uncertainty from $\cD_E$, we move back to the case when $f$ is also a GP which we denote as BLCCME-GP (Section \ref{sec: BLCME-GP}). That way we are able to incorporate both the uncertainty of $\cD_C$ and $\cD_E$.

% After that, we will consider two possible cases in estimating $\langle f, \mu_{Y|X=x}\rangle$. Finally, we will translate all of these from the conditional setting to the counterfactual one.

\subsection{Bayesian Learning of Causal Conditional Mean Embedding with KRR (BLCME-KRR)}\label{sec:BLCME-KRR}

We will start off by introducing the novel \emph{Bayesian Learning of conditional mean embedding}, followed by an extension to the causal case. 

As mentioned in section \ref{sec: background}, CMEs have a clear "feature-to-feature" regression perspective, i.e $\EE[\phi_y(Y)|X=x]$ is a result of regressing $\phi_y(Y)$ onto $\phi_x(X)$. Hence in order to account for the uncertainty when estimating on $\cD_C$, we consider a vector-valued GP construction for estimating CME. 

Consider a GP model $h(x, y)$ where $h(x, y)$ denotes $\mu_{Y|X=x}(y)$, i.e. the CME evaluated at $y$. Note that for any fixed $x$, we can recover the CME i.e $h(x,\cdot) = \mu_{Y|X=x}$. It is important to ensure that the posterior distribution of $h(x, \cdot)$ for any fixed $x\in \cX$ is restricted to $\cH_{Y}$ in order to estimate $\int f(y) p(y|X=x)dy$ via $\langle f, \mu_{Y|X=x}\rangle_{\cH_{k_y}}$. This means that we need to ensure that the samples of the V-GP of $h(x, \cdot)$ lie $\cH_{Y}$ for the inner product to be well defined. Consequently, we cannot define a $\cG\cP(0, k_x\otimes k_y)$ prior on $h$ as usual, given that the draws from such prior would almost surely fall outside $\cH_{k_x} \otimes \cH_{k_y}$ [add ref.]. Instead we follow a similar construction as in \cite{flaxman2016bayesian} and define a prior over $h$ as:
\begin{align}
    h &\sim \cG\cP(0, k_x \otimes r_y) \\
    r_y(y, y') &= \int k_y(y, u)k_y(u, y') \nu(du)
\end{align}
where $\nu$ is any finite measure on $\cY$. This choice of kernel ensures that $h \in \cH_{k_x}\otimes \cH_{k_y}$ with probability 1 by the nuclear dominance [add ref.] of $r_y$ over $k_y$ for any stationary kernel $k_y$. We follow the construction from \cite{flaxman2016bayesian} and set $\nu(du) = \exp(-\frac{||u||^2}{2\eta^2})$ where $\eta > 0$ is some hyperparameter that can be learnt along with other kernel hyperparameters using maximum likelihood in our Bayesian formulation.

The observational model is thus:
\begin{align}
    k_{y}(y_i, \cdot) = \phi_y(y_i) = h(x_i, \cdot) + \lambda^{\frac{1}{2}}\epsilon_i
\end{align}
where $\epsilon_i \sim \cG\cP(0, r)$ independently across $i$. Note that we are regressing functions on each other. By taking inner products with $\phi_y(y')$, this implies,
\begin{align}
    k_y(y_i, y') = h(x_i, y') + \lambda^{\frac{1}{2}}\epsilon_i(y')
\end{align}
The GP posterior of $h$ can thus be inferred by treating $k(y_i, y_j)$ as noisy evaluations of $h(x_i, y_j)$. 

% The resulting mean and covariance for $h$ i.e. the conditional mean embedding $\mu_{Y|X=x}(y)$ can be derived, see Proposition \label{proposition: BL-CME}.

% and hence estimate the inner product $\langle f, \mu_{Y|X=x}\rangle$.

%stacked into $vec(K_{YY})$ 

\begin{proposition}[\textbf{Bayesian Learning of Conditional Mean Embedding}] \label{proposition: BL-CME}

The posterior GP of $h(x, y) =\mu_{Y|X=x}(y)$ given the above setup has the following mean and covariance:
\begin{align}
    \bar{m}_h((x, y)) &= k(x, \bfx)(K_{\bfx\bfx} + \lambda I)^{-1}K_{\bfy\bfy}R_{\bfy\bfy}^{-1}R_{\bfy, y} \\
    \kappa_h((x, y), (x', y')) &= k_x(x,x')r_y(y, y') - k_{x\bfx}(K_{\bfx\bfx} + \lambda I)^{-1}k_{\bfx x'}r_{y\bfy}R_{\bfy\bfy}^{-1}r_{\bfy y'}
\end{align}
In addition, the following marginal likelihood can be used for hyperparameter optimisation,
\begin{align}
    \log(\PP(K_{\bfy\bfy})) = -\frac{N}{2}\Big(\log|K_{\bfx\bfx} + \lambda I| + \log|R|\Big) - \frac{1}{2}\operatorname{Tr}\Big((K_{\bfx\bfx}+\lambda I)^{-1}K_{\bfy\bfy}R_{\bfy\bfy}^{-1}K_{\bfy\bfy}\Big)
\end{align}
\end{proposition}

Now that we have derived the Bayesian conditional mean embedding it is straight forward to derive the causal version.
\begin{proposition}[\textbf{Bayesian Learning of Causal Conditional Mean Embedding}] \label{proposition: BL-CME}

The posterior GP of $\mu_{Y|do(X)=x}(y)$ given the above setup has the following mean and covariance:
\begin{align}
    m^{do}(x, y) &= \Phi_{\Omega}(x) (K_{\Omega} + \lambda I)^{-1} K_{YY} R_{YY}^{-1}R_{Y, y} \\ 
    \kappa^{do}((x, y), (x',y')) &= \Phi_{\Omega}(x)^\top \Phi_{\Omega}(x) r_y(y, y')  -\Phi_{\Omega}(x)^\top (K_{\Omega} + \lambda I)^{-1} \Phi_{\Omega}(x) R_{y,Y}R^{-1}_{YY}R_{Y, y'}
\end{align}
\end{proposition}

\textbf{Estimating the quantity of interest $\langle f, \mu_{Y|do(X)=x}\rangle_{\cH_{k_y}}$}: With the Bayesian causal CME defined, we proceed to estimate our target $\langle f, \mu_{Y|do(X)=x}\rangle$. We first consider the case when $f$ is a KRR function learnt from $\cD_E$ and later in \textsc{BLCME-GP} consider $f$ as a GP.

\jef{I think we can put this part in the appendix because noone will understand why this is important without going through the derivation}
To compute $\langle f, \mu_{Y|X=x} \rangle$ for $f \in \cH_{k_y}$, we need the following identity:
\begin{align}
    \langle f, r_y(\cdot, y) \rangle_{\cH_{k_y}} &= \Big\langle f, \int k_y(\cdot, u)k_y(u, y) \nu(du)\Big\rangle \\
    &= \int f(u)k_y(u, y)\nu(du) \\
\intertext{when $f$ is a KRR learnt from $\cD_E$, i.e $f(y) = k_{y\tilbfy}(K_{\tilbfy\tilbfy}+\lambda_f I)^{-1}\bft$, We have }
    &= \bft^\top(K_{\tilbfy\tilbfy} + \lambda_f I)^{-1}R(\tilbfy, y)
\end{align}

% Note that when $f$ is a KRR learnt from $\cD_E$ we  have that $f(y) = k_{y\tilbfy}(K_{\tilbfy\tilbfy}+\lambda_f I)^{-1}\bft$

\begin{proposition}[\textbf{Bayesian Embedding Process}]
\label{proposition: f is krr cme is gp}
Let $f$ be a KRR learnt from $\cD_E$ and we estimate $\mu_{Y|do(X)=x}$ as a GP using $\cD_C$, then the inner product $\langle f, \mu_{Y|do(X)=x}\rangle_{\cH_{k_y}}$ can be estimated using a GP with the following mean and covariance:
\begin{align}
    m_2^{do}(x) &= \Phi_{\Omega}(x) (K_{\Omega} + \lambda I)^{-1} K_{YY} R_{YY}^{-1}R_{\bfy\tilbfy} A\\
     \kappa_2^{do}(x, x') &= 
     \begin{bmatrix}
     \Phi_{\Omega}(x)^\top \Phi_{\Omega}(x) & -\Phi_{\Omega}(x')^\top (K_{\Omega} + \lambda I)^{-1} \Phi_{\Omega}(x')
     \end{bmatrix} \\
     &\quad \hspace{0.07cm}
     \begin{bmatrix}
    A^\top R_{\tilbfy\tilbfy} A & A^\top R_{\tilbfy, \bfy}R_{\bfy, \bfy}R_{\bfy, \tilbfy}A
    \end{bmatrix}^\top \nonumber
\end{align}
where $A:=(K_{\tilbfy\tilbfy} + \lambda_f I)^{-1}\bft$
\end{proposition}





% \subsubsection{Estimating $\langle f, \mu_{Y|X=x}\rangle_{\cH_{k_y}}$}
% With the Bayesian CME defined, we proceed to estimate our target $\langle f, \mu_{Y|X=x}\rangle$. We first consider the case when $f$ is a kernel ridge regression function learnt from $\cD_E$ and later consider when $f$ is itself a GP, so as to incorporate this extra uncertainty into our estimation. 

% \subsubsection{$f$ is a Kernel Ridge Regression}
% To compute $\langle f, \mu_{Y|X=x} \rangle$ for $f \in \cH_{k_y}$, we need to be able to compute $\langle f, r_y(\cdot, y) \rangle_{\cH_{k_y}}$, which corresponds to
% \begin{align}
%     \langle f, r_y(\cdot, y) \rangle_{\cH_{k_y}} &= \Big\langle f, \int k_y(\cdot, u)k_y(u, y) \nu(du)\Big\rangle \\
%     &= \int f(u)k_y(u, y)\nu(du) \\
% \intertext{when $f$ is a KRR learnt from $\cD_E$, i.e $f(y) = k_{y\tilbfy}(K_{\tilbfy\tilbfy}+\lambda_f I)^{-1}\bft$, We have }
%     &= \bft^\top(K_{\tilbfy\tilbfy} + \lambda_f I)^{-1}R(\tilbfy, y)
% \end{align}
% With this we have the following proposition,
% \begin{proposition}
% \label{proposition: f is krr cme is gp}
% Let $f$ be a KRR learnt from $\cD_E$ and we estimate $\mu_{Y|X=x}$ as a GP using $\cD_C$, then the inner product $\langle f, \mu_{Y|X=x}\rangle_{\cH_{k_y}}$ can be estimated using a GP with the following mean and covariance:
% \begin{align}
%     m_2(x) &= k_{x\bfx}(K_{\bfx\bfx} + \lambda I)^{-1}K_{\bfy\bfy}R_{\bfy\bfy}^{-1}R_{\bfy\tilbfy} A \\
%     \kappa_2(x, x') &= 
%     \begin{bmatrix}
%     k_{xx'} & -k_{x\bfx}(K_{\bfx\bfx} + \lambda I)^{-1}k_{\bfx x'}
%     \end{bmatrix}
%     \begin{bmatrix}
%     A^\top R_{\tilbfy\tilbfy} A & A^\top r_{\tilbfy, \bfy}R_{\bfy, \bfy}r_{\bfy, \tilbfy}A
%     \end{bmatrix}^\top
% \end{align}
% where $A:=(K_{\tilbfy\tilbfy} + \lambda_f I)^{-1}\bft$
% \end{proposition}

% \subsection{\textsc{CASE 3}: Estimate $f$ using a GP and $\mu_{Y|do(X)=x}$ using V-GP}
% Lastly, to incorporate both uncertainties in $\cD_C$ and $\cD_E$, we estimate $\langle f, \mu_{Y|X=x} \rangle_{\cH_{k_y}}$ by setting both $f$ and $\mu_{Y|X=x}$ as GPs. However, we again need to ensure $f$ is supported on $\cH_{k_y}$, hence we put a $\cG\cP(0, r_y)$ prior on $f$. In fact, under this construction, we have an alternative way of expressing the posterior $f|\bft$:
% \begin{proposition}[Induced distribution on $f$]\label{proposition: induced dist on f}
% Let $\hat{\bfy} = [\bfy^\top \hspace{0.1cm} \tilbfy^\top]^\top$ be the concatenation of $\bfy$ and $
% \tilbfy$. The nuclear dominant kernel formulation induces the following posterior distribution on $f$,
% \begin{align}
%     f|\bft \sim N\big(\Phi_{\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1}R_{\hat{\bfy}\tilbfy}(R_{\tilbfy\tilbfy} + \lambda_f I)^{-1}\bft, \Phi_{\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1} \bar{R}_{\hat{\bfy}\hat{\bfy}} K_{\hat{\bfy}\hat{\bfy}}^{-1} \Phi_{\hat{\bfy}}^\top\big)
% \end{align}
% where $\bar{R}_{\hat{\bfy}\hat{\bfy}} = R_{\hat{\bfy}\hat{\bfy}} - R_{\hat{\bfy}\tilbfy}(R_{\tilbfy\tilbfy} + \lambda_f I)^{-1} R_{\tilbfy\hat{\bfy}}$.
% \end{proposition}
% Similarly for $\mu_{Y|X=x} = h(x, \cdot)$,
% \begin{proposition}[Induced distribution on $\mu_{Y|X=x}$]\label{proposition: induced dist on mu}
% The nuclear dominant kernel formulation induces the following distribution on $h(x, \cdot)$,
% \begin{align}
%     h(x, \cdot)|K_{\bfy\bfy} \sim N\big(\Phi_{\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1}R_{\hat{\bfy}\bfy}R_{\bfy\bfy}^{-1}K_{\bfy \bfy}(K_{\bfx\bfx} + \lambda I)^{-1}k_{\bfx x}, \Phi_{\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1}K^{h_x}_{\hat{\bfy}\hat{\bfy}} K_{\hat{\bfy}\hat{\bfy}}^{-1}\Phi_{\hat{\bfy}}\big)
% \end{align}
% where $K^{h_x}_{\hat{\bfy}\hat{\bfy}} = k_{xx}R_{\hat{\bfy}\hat{\bfy}} - \big(k_{x\bfx}(K_{\bfx\bfx}+\lambda I)^{-1}k_{\bfx x}\big) R_{\hat{\bfy}\bfy} (R_{\bfy\bfy}+\lambda I)^{-1}R_{\bfy\hat{\bfy}}$
% \end{proposition}
% Now $\langle f, \mu_{Y|X=x} \rangle$ becomes an inner product between two independent (learnt from two independent datasets) infinite dimensional Gaussian vector, thus we have the following,
% \begin{proposition}\label{proposition: case 3}
% Let $f$ and $\mu_{Y|X=x}$ be GPs learnt with the above setup, then the inner product $\langle f, \mu_{Y|X=x} \rangle$ can be estimated using a GP on $x$ with the following mean and covariance,
% \begin{align}
% \smallfont
%     m_3(x) &= k_{x\bfx}(K_{\bfx\bfx} + \lambda I)^{-1}K_{\bfy\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1}R_{\hat{\bfy}\tilbfy}(R_{\tilbfy\tilbfy} + \lambda_f I)^{-1} \bft \\
%     \kappa_3(x, x') &= k_{x\bfx}(K_{\bfx\bfx} + \lambda I)^{-1}\Theta_1^\top \bar{R}_{\hat{\bfy}\hat{\bfy}} \Theta_1 (K_{\bfx\bfx} + \lambda I)^{-1} k_{\bfx x'} \\ 
%     &\quad + [k_{xx'} \quad -k_{x\bfx}(K_{\bfx\bfx} + \lambda I)^{-1}k_{\bfx x'}][\Theta_2 \quad \Theta_3]^\top
% \end{align}
% where $\Theta_1 = K_{\hat{\bfy}\hat{\bfy}}^{-1}R_{\hat{\bfy}\bfy}R_{\bfy\bfy}^{-1}K_{\bfy\bfy}$, $\Theta_2 = \Theta_4^\top R_{\hat{\bfy}\hat{\bfy}}\Theta_4$, $\Theta_3 = \Theta_4^\top R_{\hat{\bfy}\bfy}R_{\bfy\bfy}^{-1}R_{\bfy\hat{\bfy}}\Theta_4$ and $\Theta_4 = K_{\hat{\bfy}\hat{\bfy}}R_{\hat{\bfy}\tilbfy}(K_{\tilbfy\tilbfy}+\lambda_f)^{-1}\bft$.
% \end{proposition}


\subsection{Bayesian Learning of (Causal) Conditional Mean Embedding with GP (BLCME-GP)}\label{sec: BLCME-GP}
Lastly, to incorporate both uncertainties in $\cD_C$ and $\cD_E$, we estimate $\langle f, \mu_{Y|X=x} \rangle_{\cH_{k_y}}$ by setting both $f$ and $\mu_{Y|X=x}$ as GPs. However, we again need to ensure $f$ is supported on $\cH_{k_y}$, hence we put a $\cG\cP(0, r_y)$ prior on $f$. Note that the resulting quantity from the inner product is in fact not a Gaussian anymore. However, since the target integral is Gaussian itself, we will match the first two moment by estimating the mean and covariance from $\langle f, \mu_{Y|do(X)=x} \rangle$. Due to this we simply added this case for completeness and used mainly a combination of \textsc{Causal Mean Process} and \textsc{BLCME-KRR} which we will elaborate on in our experiment section

\begin{proposition}[\textbf{Fully Bayesian Mean Embedding Process}]\label{proposition: STAGE 3}
Let $f$ and $\mu_{Y|X=x}$ be GPs learnt with the above setup, then the inner product $\langle f, \mu_{Y|X=x} \rangle$ can be estimated using a GP on $x$ with the following mean and covariance,
\begin{align}
\smallfont
    m_3^{do}(x) &= \Phi_{\Omega}(x) (K_{\Omega} + \lambda I)^{-1}K_{\bfy\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1}R_{\hat{\bfy}\tilbfy}(R_{\tilbfy\tilbfy} + \lambda_f I)^{-1} \bft \\
    \kappa_3(x, x') &= \Phi_{\Omega}(x) (K_{\Omega} + \lambda I)^{-1}\Theta_1^\top \bar{R}_{\hat{\bfy}\hat{\bfy}} \Theta_1  (K_{\Omega} + \lambda I)^{-1} \Phi_{\Omega}(x') \\ 
    &\quad + \begin{bmatrix}
     \Phi_{\Omega}(x)^\top \Phi_{\Omega}(x') & -\Phi_{\Omega}(x)^\top (K_{\Omega} + \lambda I)^{-1} \Phi_{\Omega}(x')
     \end{bmatrix} [\Theta_2 \quad \Theta_3]^\top
\end{align}
where $\Theta_1 = K_{\hat{\bfy}\hat{\bfy}}^{-1}R_{\hat{\bfy}\bfy}R_{\bfy\bfy}^{-1}K_{\bfy\bfy}$, $\Theta_2 = \Theta_4^\top R_{\hat{\bfy}\hat{\bfy}}\Theta_4 + tr(K_{\hat{\bfy}, \hat{\bfy}}^{-1}R_{\hat{\bfy}\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1}\bar{R}_{\hat{\bfy}\hat{\bfy}})$, $\Theta_3 = \Theta_4^\top R_{\hat{\bfy}\bfy}R_{\bfy\bfy}^{-1}R_{\bfy\hat{\bfy}}\Theta_4 + tr(R_{\hat{\bfy}\bfy}R_{\bfy\bfy}^{-1}R_{\bfy\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1}\bar{R}_{\hat{\bfy}\hat{\bfy}}K_{\hat{\bfy}\hat{\bfy}}^{-1})$ and $\Theta_4 = K_{\hat{\bfy}\hat{\bfy}}^{-1}R_{\hat{\bfy}\tilbfy}(K_{\tilbfy\tilbfy}+\lambda_f)^{-1}\bft$.
\end{proposition}

We note that the uncertainty $\kappa_3$ consists of 3 separate parts, while the first one considers uncertainty from $f$, similar to \textsc{Causal Conditional Mean Process}, whereas a second term that utilise the uncertainty from estimating $\mu_{Y|do(X)=x}$, similar to $\textsc{BLCME-KRR}$, with an extra trace term that can be interpret as an interaction of the two uncertainties.

==> 99_paper_figs/05_discussion.tex <==
\section{Discussion and possible extensions}
The main object of interest here:
\begin{align}
    \mathbb{E}[X_{p+1}|do(X_0)=x_0]
\end{align}
is there a way to incorporate the uncertainty across the graphs and reason about the object of interest? In other words, is the above expectation identifiable? The answer is yes.
\begin{align}
    \mathbb{E}[X_{p+1}|do(X_0)=x_0] &= \int \mathbb{E}[X_{p+1}|X_p, Z_p]p(Z_p) p(dX_{p}|do(X_0)=x_0) \\
    &\approx \int f(X_p, Z_p) p(dZ_p)p(dX_{p}|do(X_0) = x_0)
\end{align}

and now we will show by induction one can represent the expectation as a chain of embeddings.

When $p=1$, we can represent $\mathbb{E}[X_2|do(X_0)=x_0]$ as,
\begin{align}
    \mathbb{E}[X_2|do(X_0)=x_0] &\approx \int f(X_1, Z_1) p(dZ_1)p(dX_1|do(X)=x_0) \\
    &= \langle f, C_{\ddot{X}_1|do(X_0)} \rangle
\end{align}
where we set $\ddot{X}_1 =X_1, Z_1$ and define. 

THIS 
\begin{align}
    \mathbb{E}[X_2|do(X_0)=x_0] &\approx {\bf f}^\top(K_{\ddot{X}} + \lambda I)^{-1}\Phi_{\ddot{X}}^\top (\mu_{Z_1} \otimes \mu_{X_1|do(X)=x_0})
\end{align}

and we know we can define the do embedding $\mu_{X_1|do(X)=x_0}$ from existing work. 
\begin{align}
    \mu_{X_1|do(X_0)=x_0} &= \int \phi(x_1) dP(x_1|do(X_0) = x_0) \\
                          &= \int\int \phi(x_1) p(dx_1|X_0=x_0, Z_0=z_0) p(dz_0) \\
                          &\approx \int \hat{C}_{X_1|X_0, Z_0} (k_{X_0}(x_0, \cdot) \otimes k_{Z_0}(z_0, \cdot) ) p(dz_0)\\
    &= \hat{C}_{X_1|Z_0,X_0} (\mu_{Z_0} \otimes k_{X_0}(x_0, \cdot))
\end{align}

So the key in the induction process is to show we can identify $\mu_{X_p|do(X_0)=x_0}$, but this is,
\begin{align}
    \mu_{X_p|do(X_0)=x_0} &= \int \phi_{X_p}p(dX_{p}|do(X_0)=x_0) \\
    &= \int \int \phi_{X_p} p(X_p|Z_{p-1}, X_{p-1})p(dZ_{p-1})p(dX_{p-1}|do(X_0)=x_0) \\
    &= C_{X_p|\ddot{X}_{p-1}} (\mu_{Z_{p-1}} \otimes \mu_{X_{p-1}|do(X_0)=x_0})
\end{align}
therefore if we know $\mu_{X_1|do(X_0)=x_0}$, then by induction, we can know $\mu_{X_p|do(X_0)=x_0}$, and because of that, we can estimate $\mathbb{E}[X_p|do(X_0)=x_0]$.

Now the next question is, can we also incorporate the uncertainty quantification techniques we developed for Causal Mechanism v.s. Experimental in this chained setting? Recall we can express,
\begin{align}
    \mathbb{E}[X_{p+1}|do(X_0) = x_0] = \langle f, C_{\ddot{X_p}|do(X_0)=x_0} \rangle
\end{align}
From the above, since we have an identifiable closed form solution as operators for $C_{\ddot{X}_{p}|do(X_0)=x_0}$, therefore if $f$ is a GP, we can still apply the probabilistic integration techniques.

What about when $f$ is KRR and the embedding is uncertain? What can we do? In fact there is some modelling choice we have to make. Recall $\mu_{X_1|do(X_0)=x_0}$ can be written as a GP that is defined on $X_0$ and output stuff in $\mathcal{H}_{X_1}$

